GF + MMT = GLF -- From Language to Semantics through LF

These days, vast amounts of knowledge are available online, most of it in written form. Search engines help us access this knowledge, but aggregating, relating and reasoning with it is still a predominantly human effort. One of the key challenges for automated reasoning based on natural-language texts is the need to extract meaning (semantics) from texts. Natural language understanding (NLU) systems describe the conversion from a set of natural language utterances to terms in a particular logic. Tools for the co-development of grammar and target logic are currently largely missing. We will describe the Grammatical Logical Framework (GLF), a combination of two existing frameworks, in which large parts of a symbolic, rule-based NLU system can be developed and implemented: the Grammatical Framework (GF) and MMT. GF is a tool for syntactic analysis, generation, and translation with complex natural language grammars and MMT can be used to specify logical systems and to represent knowledge in them. Combining these tools is possible, because they are based on compatible logical frameworks: Martin-L\"of type theory and LF. The flexibility of logical frameworks is needed, as NLU research has not settled on a particular target logic for meaning representation. Instead, new logics are developed all the time to handle various language phenomena. GLF allows users to develop the logic and the language parsing components in parallel, and to connect them for experimentation with the entire pipeline.

==> eptcsdata.tex <==
\providecommand{\firstpage}{24}
\providecommand{\publicationstatus}{D. Miller, I. Scagnetto (Eds.)\\
Logical Frameworks and Meta-Languages:\\
Theory and Practice 2019 (LFMTP 2019)\\
EPTCS 307, 2019, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{http://dx.doi.org/10.4204/EPTCS.307.4}{10.4204/EPTCS.307.4}}


==> pgflibrarytikzmmt.code.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% A TIKZ library for MMT Theory Graphs
% copyright 2014 Michael Kohlhase; Released under the LPPL
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
% this library provides some standardized node and arrow styles for formatting MMT graph
% diagrams in tikz. The advantage is that we can classify the arrows and nodes
% symbolically and with the styles in this library achieve a uniform look that helps
% readability. 
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%% 1. Theories
% a generic theory
\def\outerthysep{.3mm}
\def\innerthysep{.5mm}
\tikzstyle{thy}=[draw,outer sep=\outerthysep,rounded corners,inner sep=\innerthysep]
% a primitive theory
\tikzstyle{primthy}=[thy,double]
% a theory graph 
\tikzstyle{thygraph}=[draw,outer sep=1mm,rounded corners,dashed]

%%% 2. Arrows 
%%% 2.1. Arrowtips (only internal)
\usetikzlibrary{arrows}
\newcommand{\@mmtarrowtip}{angle 45}
\newcommand{\@mmtreversearrowtip}{angle 45 reversed}
\newcommand{\@mmtarrowtipepi}{triangle 45}
\newcommand{\@mmtarrowtipmonoright}{right hook}
\newcommand{\@mmtarrowtipmonoleft}{left hook}
\newcommand{\@mmtarrowtippartial}{right to}
\newcommand{\@mmtarrowtippartialleft}{left to}
\newcommand{\@mmtreversearrowtippartial}{right to reversed}
\newcommand{\@mmtreversearrowtippartialleft}{left to reversed}

%%% 2.2 the arrow sstyles in graphs
\usetikzlibrary{decorations,decorations.pathmorphing,decorations.markings}
% any morphism 
\tikzstyle{morph}=[-\@mmtarrowtip,thick] 
\tikzstyle{mapsto}=[|-\@mmtarrowtip] %| any morphism 
% structures
\tikzstyle{struct}=[-\@mmtarrowtip,thick]
% inclusions: regular, partial, and left variants
\tikzstyle{include}=[\@mmtarrowtipmonoright-\@mmtarrowtip,thick]
\tikzstyle{revinclude}=[\@mmtarrowtip-\@mmtarrowtipmonoright,thick]
\tikzstyle{pinclude}=[\@mmtarrowtipmonoright-\@mmtarrowtippartial,thick]
\tikzstyle{includeleft}=[\@mmtarrowtipmonoleft-\@mmtarrowtip,thick]
\tikzstyle{pincludeleft}=[\@mmtarrowtipmonoleft-\@mmtarrowtippartialleft,thick]
% views: regular, mono, partial, and left variants
\tikzstyle{preview}=[decorate,
                                decoration={coil,aspect=0,amplitude=1pt,
                                                    segment length=6pt,
                                                    pre=lineto,pre length=3pt,
                                                    post=lineto,post length=5pt},
                                thick]
\tikzstyle{view}=[preview,-\@mmtarrowtip]
\tikzstyle{mview}=[preview,\@mmtarrowtipmonoright-\@mmtarrowtip]
\tikzstyle{pview}=[preview,-\@mmtarrowtippartial]
\tikzstyle{pmview}=[preview,\@mmtarrowtipmonoright-\@mmtarrowtippartial]
\tikzstyle{viewleft}=[preview,-\@mmtarrowtip]
\tikzstyle{mviewleft}=[preview,\@mmtarrowtipmonoleft-\@mmtarrowtip]
\tikzstyle{pviewleft}=[preview,-\@mmtarrowtippartialleft]
\tikzstyle{pmviewleft}=[preview,\@mmtarrowtipmonoleft-\@mmtarrowtippartialleft]
\tikzstyle{adoption}=[preview,thin,double,-\@mmtarrowtip]
% biviews: regular, partial, and left variants
\tikzstyle{biview}=[preview,\@mmtarrowtip-\@mmtarrowtip]
\tikzstyle{pbiview}=[preview,\@mmtreversearrowtippartial-\@mmtarrowtippartial]
\tikzstyle{pbiviewleft}=[preview,\@mmtreversearrowtippartialleft-\@mmtarrowtippartialleft]
% defining views (experimental)
\tikzstyle{defview}=[preview,densely dotted,-\@mmtarrowtip]
% meta-theory inclusion
\tikzstyle{meta}=[dotted,-\@mmtarrowtip,thick]
% conservative extensions (abbreviation)
\tikzstyle{conservative}=[hooks-\@mmtarrowtip,double] 
% conservative development
\tikzstyle{conservdev}=[hooks-\@mmtarrowtip,dashed,double] 

% antimorphisms as striktthroughs
\tikzset{anti/.style={
    decoration={markings, mark=between positions 0.2 and 0.8 step 4mm with {
        \draw [thick,-] ++ (-3pt,-3pt) -- (3pt,3pt);}},
    postaction={decorate}}}

% parallel markup
\tikzstyle{parallel}=[\@mmtarrowtip-\@mmtarrowtip,dashed]

%%%% 3. Realms 
\tikzstyle{prerealm}=[draw=blue!40,rectangle,rounded corners,inner sep=10pt,inner ysep=20pt]
\tikzstyle{realm}=[prerealm,fill=gray!4]
\tikzstyle{pillar}=[prerealm,fill=gray!10]

%%% 4. convenience macros
%%% 4.1 the \mmtthy macro takes three arguments, name, decl, axioms and makes a 
% table-like structure
\newcommand\mmtthy[3]{\def\@second{#2}\def\@third{#3}%
\begin{array}{l}\textsf{#1}%
\ifx\@second\@empty\else\\\hline #2\fi%
\ifx\@third\@empty\else\\\hline #3\fi%
\end{array}}
%%% 4.2 the \mmtar takes two arguments, some tikz options, and an arrow style. \nmmtar
% is a variant that also has a name on top.
\newcommand\mmtar[2][]{\raisebox{.5ex}{\tikz[#1]{\draw[#2] (0,0) -- (.6,0);}}}
\newcommand\nmmtar[3][]{\raisebox{.4ex}{\tikz[#1]{\draw[#2] (0,0) --
      node[above]{\ensuremath{\scriptstyle #3}} (.8,0);}}}
%%%% 3.3 Pushout symbols
%%  (after http://tex.stackexchange.com/questions/1144/pushouts-and-pullbacks)
%% \nepushout[<pos>]{<basenode>}{<targetnode>} positions a pushout symbol 
%% (available separately as \pushoutsymb) <pos> of the way between <basenode>
%%  and <targetnode>. 
\usetikzlibrary{calc}
\newcommand\@pushout[4][]{\def\@test{#1}%
\ifx\@test\@empty\def\@@num{.5}\else\def\@@num{#1}\fi%
\begin{scope}[shift=($(#2)!\@@num!(#3)$)]\@nameuse{@#4pushoutsymb}\end{scope}} 
\newcommand\@nepushoutsymb{\draw +(-.2,0) -- +(0,0)  -- +(0,-.2);\fill +(-.1,-.1) circle (.03);}
\newcommand\nepushoutsymb{\tikz{\@nepushoutsymb}}
\newcommand\nepushout[3][]{\@pushout[#1]{#2}{#3}{ne}}

\newcommand\@sepushoutsymb{\draw +(-.2,0) -- +(0,0)  -- +(0,.2);\fill +(-.1,.1) circle (.03);}
\newcommand\sepushoutsymb{\tikz{\@sepushoutsymb}}
\newcommand\sepushout[3][]{\@pushout[#1]{#2}{#3}{se}}

\newcommand\@nwpushoutsymb{\draw +(.2,0) -- +(0,0)  -- +(0,-.2);\fill +(.1,-.1) circle (.03);}
\newcommand\nwpushoutsymb{\tikz{\@nwpushoutsymb}}
\newcommand\nwpushout[3][]{\@pushout[#1]{#2}{#3}{nw}}

\newcommand\@swpushoutsymb{\draw +(.2,0) -- +(0,0)  -- +(0,.2);\fill +(.1,.1) circle (.03);}
\newcommand\swpushoutsymb{\tikz{\@swpushoutsymb}}
\newcommand\swpushout[3][]{\@pushout[#1]{#2}{#3}{sw}}

\newcommand\@npushoutsymb{\draw +(-.1,-.1) -- +(0,0)  -- +(.1,-.1);\fill +(0,-.1) circle (.03);}
\newcommand\npushoutsymb{\tikz{\@npushoutsymb}}
\newcommand\npushout[3][]{\@pushout[#1]{#2}{#3}{n}}

\newcommand\@spushoutsymb{\draw +(-.1,.1) -- +(0,0)  -- +(.1,.1);\fill +(0,.1) circle (.03);}
\newcommand\spushoutsymb{\tikz{\@spushoutsymb}}
\newcommand\spushout[3][]{\@pushout[#1]{#2}{#3}{s}}

\newcommand\@wpushoutsymb{\draw +(-.1,-.1) -- +(0,0)  -- +(-.1,.1);\fill +(-.1,0) circle (.03);}
\newcommand\wpushoutsymb{\tikz{\@wpushoutsymb}}
\newcommand\wpushout[3][]{\@pushout[#1]{#2}{#3}{w}}

\newcommand\@epushoutsymb{\draw +(.1,.1) -- +(0,0)  -- +(.1,-.1);\fill +(.1,0) circle (.03);}
\newcommand\epushoutsymb{\tikz{\@epushoutsymb}}
\newcommand\epushout[3][]{\@pushout[#1]{#2}{#3}{e}}

%%%%%% testing them: 
% \begin{tikzpicture}[scale=1.5]
%   \node (a) at (0,0) {a};
%   \node (b) at (1,0) {b};
%   \node (c) at (1,1) {c};
%   \node (d) at (0,1) {d};
%   \nepushout[.8]{a}c;
%   \nwpushout[.8]{b}d;
%   \sepushout[.8]{d}b;
%   \swpushout[.8]{c}a;
%   \draw (a) -- (b) -- (c) -- (d) -- (a);
%   \node (aa) at (4,0) {a};
%   \node (bb) at (3.5,.5) {b};
%   \node (cc) at (4,1) {c};
%   \node (dd) at (4.5,.5) {d};
%   \draw (aa) -- (bb) -- (cc) -- (dd) -- (aa);
%   \npushout[.8]{aa}{cc};
%   \spushout[.8]{cc}{aa};
%   \wpushout[.8]{bb}{dd};
%   \epushout[.8]{dd}{bb};
% \end{tikzpicture}

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "test"
%%% End:


==> tikzlibrarymmt.code.tex <==
\input{pgflibrarytikzmmt.code.tex}

